Optimal Investment and Entropy-Regularized Learning Under Stochastic Volatility Models with Portfolio Constraints

We study the problem of optimal portfolio selection under stochastic volatility within a continuous time reinforcement learning framework with portfolio constraints. Exploration is modeled through entropy-regularized relaxed controls, where the investor selects probability distributions over admissible portfolio allocations rather than deterministic strategies. Using dynamic programming arguments, we derive the associated entropy-regularized Hamilton-Jacobi-Bellman equation, whose Hamiltonian involves optimization over probability measures supported on a compact control set. We show that the optimal exploratory policy takes the form of a truncated Gaussian distribution characterized by spatial derivatives of the solution of the resulting nonlinear quasilinear parabolic partial differential equation. Under suitable structural conditions on the model coefficients, we prove the existence of classical solutions to this nonlinear HJB equation for the value function. We then establish a verification theorem and analyze the policy-improvement structure induced by the entropy-regularized Hamiltonian, showing how the resulting sequence of PDEs provides a continuous-time interpretation of actor-critic learning dynamics. Finally, our PDE analysis with a semi-closed form of optimal value and optimal policy enables the design of an implementable reinforcement learning algorithm by recasting the optimal problem in a martingale framework.

==> tab_bias.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Effect of exploration on the mean weight when the cap binds ($\eta=0.7$, $b=1$, $t=0$): $-\partial_m\mathbb{E}[\lambda^{*}]$ computed from the reduced equation (measured) and from Corollary 1 (closed form).}
\label{tab:bias}
\begin{tabular}{lrrrr}
\hline
$\sigma(y)$ & $\alpha^{*}$ & measured & closed form & relative gap \\
\hline
0.061 & 9.280 & 45.74 & 45.75 & -0.02\% \\
0.082 & 7.921 & 30.55 & 30.55 & -0.02\% \\
0.109 & 6.626 & 21.35 & 21.35 & -0.02\% \\
0.144 & 5.547 & 15.16 & 15.16 & -0.01\% \\
0.186 & 4.724 & 11.13 & 11.13 & -0.01\% \\
0.233 & 4.109 & 8.50 & 8.50 & -0.01\% \\
0.296 & 3.549 & 6.38 & 6.38 & -0.01\% \\
\hline
\end{tabular}
% \begin{minipage}{\linewidth}\vspace{2mm}\footnotesize The agreement is within three tenths of a percentage point across the whole volatility range. The coefficient does not vanish at $\rho=0$ and grows as volatility falls, because the market price of risk stays bounded away from zero while $\sigma(y)$ falls to its floor $\sigma_*$; exploration therefore pulls the implemented weight away from the boundary most strongly in calm markets --- which are, by \eqref{eq:num-par}, exactly the states in which the cap binds.\end{minipage}
\end{table}
